Data Curation with Deep Learning [Vision]

Data curation - the process of discovering, integrating, and cleaning data - is one of the oldest, hardest, yet inevitable data management problems. Despite decades of efforts from both researchers and practitioners, it is still one of the most time consuming and least enjoyable work of data scientists. In most organizations, data curation plays an important role so as to fully unlock the value of big data. Unfortunately, the current solutions are not keeping up with the ever-changing data ecosystem, because they often require substantially high human cost. Meanwhile, deep learning is making strides in achieving remarkable successes in multiple areas, such as image recognition, natural language processing, and speech recognition. In this vision paper, we explore how some of the fundamental innovations in deep learning could be leveraged to improve existing data curation solutions and to help build new ones. In particular, we provide a thorough overview of the current deep learning landscape, and identify interesting research opportunities and dispel common myths. We hope that the synthesis of these important domains will unleash a series of research activities that will lead to significantly improved solutions for many data curation tasks.

==> old-sec-neuralps.tex <==
%!TEX root = main.tex

\section{Data Curation by \\ Neural Program Synthesis}
\label{subsec:ps}

So far, our discussion has been limited to traditional DC problems with simple outputs.
Oftentimes, DC desires more complicated output such as a program (for ETL scripts) or a graph (for data violations). 
However, DL models for structured output are still in infancy. 
%
In what follows, we will discuss 
how to build DL models for more complex DC problems where the output is a program.
%the automatic generation of programs for more complex DC problems.

The area of program synthesis aims to \emph{automatically construct programs}, in a programming or domain specific language (DSL), 
that  are consistent with some specification - as a formal specification but often through few input-output examples.
For example, given the input-output specification \{(John Smith, J Smith), (Jane Doe, J Doe), $\ldots$,\},
Flashfill~\cite{DBLP:conf/popl/Gulwani11} can construct a program based on Excel's macros that can perform a regular expression based string transformation.
Program synthesis is often very challenging as it requires searching over the space of all possible programs 
in the programming language that satisfies the input-output examples.
Recently, there has been extensive interest in applying DL for program synthesis.
This often takes the form of \emph{neural program synthesis}~\cite{balog2016deepcoder,parisotto2016neuro} where a neural network is trained 
on input-output examples and generates a program.
An alternate approach is \emph{neural program induction}~\cite{DBLP:journals/ercim/KurachAS16,DBLP:journals/corr/NeelakantanLS15} where the neural network produces outputs for new inputs by using a latent specification 
of the program without explicitly generating it.
One can see that this area can be very promising for DC.

\subsubsection*{\ding{45} Research Opportunities}

\begin{itemize}
    \item \emph{Syntactic and Semantic Transformations.}
        Flashfill~\cite{DBLP:conf/popl/Gulwani11} can be used for regular expression driven string transformation from input-output examples.
        How can one extend such a method to perform more sophisticated string transformations that are not constrained by regular expressions as a DSL?
        How can one further extend these to perform semantic transformations~\cite{DBLP:conf/icde/AbedjanMIOPS16}? 
        For instance, given the example pairs, \{(France, Paris), (Germany, Berlin), $\ldots$, \} can one automatically learn that 
        the latter is the capital city of the former?
    \item \emph{Domain Specific Language for Data Curation.}
        Program synthesis often searches for valid programs within the confines of a DSL, such as regular expressions.
        Is it possible to come up with a DSL that can encode common DC operations?
        This can dramatically simplify the coding and debugging code for common data cleaning and wrangling operations.
    \item \emph{Program Synthesis from ETL Scripts.}
        Currently, program synthesis is restricted to simple DSLs such as regular expressions.
        Often, enterprises have a number of pre-written ETL scripts.
        How can program synthesis be used to generate such ETL scripts automatically?
        Consider an example where we wish to integrate two relations.
        If we give a set of input-output tuples, is it possible to identify a series of ETL operations that can generate this virtual relation automatically?
    \item \emph{Interactive and Preference-driven Program Synthesis.}
        In a number of cases, the input-output is provided in an interactive manner by the domain expert.
        How can one learn the intrinsic preferences of the domain expert and use it to identify the appropriate program for the given input-output examples.
        As an example, consider the entity consolidation problem~\cite{deng2017entity}, 
        where a group of tuples that refer to the same underlying entity are consolidated by selecting the appropriate value for each attribute.
        Given conflicting values ``John Smith'' and ``J Smith'' for the attribute Name, the domain expert might prefer to use the former to latter.
        Can one use program synthesis to identify the preferences of the domain expert 
        so as to automatically take them into account for other conflicting tuples?
\end{itemize}

